Numerical Electromagnetic Frequency Domain Analysis with Discrete Exterior Calculus

In this paper, we perform a numerical analysis in frequency domain for various electromagnetic problems based on discrete exterior calculus (DEC) with an arbitrary 2-D triangular or 3-D tetrahedral mesh. We formulate the governing equations in terms of DEC for 3D and 2D inhomogeneous structures, and also show that the charge continuity relation is naturally satisfied. Then we introduce effective signed dual volume to incorporate material information into Hodge star operators and take into account the case when circumcenters fall outside triangles or tetrahedrons, which may lead to negative dual volume without Delaunay triangulation. Then we demonstrate the implementation of various boundary conditions, including perfect magnetic conductor (PMC), perfect electric conductor (PEC), Dirichlet, periodic, and absorbing boundary conditions (ABC) within this method. An excellent agreement is achieved through the numerical calculation of several problems, including homogeneous waveguides, microstructured fibers, photonic crystals, scattering by a 2-D PEC, and resonant cavities.

==> shortcuts16.tex <==
%Defination for shortcuts for commands;
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\hatb}[1]{{\hat{\bf #1}}}
\renewcommand{\v}[1]{{{\mathaccent #1}}}
\renewcommand{\c}[1]{{{\mathcal #1}}}
\newcommand{\dyad}[1]{\mbox{$\overline{ \v{#1} }$}}
\newcommand{\lagr}{\mbox{\boldmath $\lambda$}}
\newcommand{\intsol}{\mbox{\boldmath $\phi$}}
\newcommand{\rhov}{\mbox{\boldmath $\rho$}}
\newcommand{\tr}{{\dagger}}
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\dd}[2]{\frac{\text{d} #1}{\text{d} #2}}
\newcommand{\od}[2]{\frac{d #1}{d #2}}
\newcommand*{\ts}[1]{\overline{\overline{#1}}}
\newcommand{\funcd}[2]{\frac{\delta #1}{\delta #2}}

\newcommand{\commuteo}[2]{{\left[\hat #1,\hat #2\right]}}

%\renewcommand{\hatv}[1]{{\hat{\bf #1}}}


\def\hatv #1{\hat{\v{#1}}}
\def\WRT{with respect to}
\def\IBP{integration by parts}
\def\CR{commutation relation}

\def\ED{\end{document}}



\def\dyad #1{\v{\overline{#1}}}
\def\dyadg #1{{\boldsymbol{\overline{#1}}}}
\def\vE{\v E}
\def\vH{\v H}
\def\vD{\v D}
\def\vB{\v B}

%boldface greek

\newcommand{\vg} [1]{\mbox{\boldmath $#1$}}
\newcommand{\hatvg} [1]{\hat{\mbox{\boldmath $#1$}}}

\newcommand{\scriptl}{$\mathbb{L}$}


\def\be{\begin{equation} }
\def\ee{\end{equation} }

\def\domain #1{D(\mathbb{#1})}
\def\range #1{R(\mathbb{#1})}

\def\vromega{(\v r, \omega)}

\newcount\timehh\newcount\timemm
\timehh=\time \divide\timehh by 60 \timemm=\time \count255=\timehh
\multiply\count255 by -60 \advance\timemm by \count255
\def\draftheader{\slshape\today\ at
\ifnum\timehh<10 0\fi\number\timehh\,:\,\ifnum\timemm<10 0\fi\number\timemm}%


\def\norm #1{\left\| {#1} \right\|}

\def\Krylov#1{\mathcal K^{#1}\left(\dyad A,\v r_0\right)}



\newcommand{\jeq}{\mathbf J_{eq}}
\newcommand{\rbar}{(\mathbf r)}
\newcommand{\rbarp}{(\mathbf r')}
\newcommand{\bg}{\mathbf{\overline G}}
\newcommand{\prs}{(\mathbf r, \mathbf r')}
\newcommand{\meq}{\mathbf M_{eq}}
\newcommand{\hinc}{\mathbf H_{inc}}
\newcommand{\einc}{\mathbf E_{inc}}

\def\tdot{\hat t\cdot}
\def\Itd{\dyad I_t\cdot}
\def\It{\dyad I_t}

\newcommand{\js}{\mathbf J_{s}}
\newcommand{\bt}{\mathbf T}
\newcommand{\bbf}{\mathbf F}
\newcommand{\bmu}{\boldsymbol{\overline{\mu}}}
\newcommand{\beps}{\boldsymbol{\overline{\epsilon}}}
\newcommand{\bbtau}{\boldsymbol{\overline{\tau}}}
\newcommand{\bbI}{{\bf\overline{I}}}
\newcommand{\bbg}{\mathbf{\overline G}}
\newcommand{\bbi}{{\bf\overline I}}

\newcommand{\jays}{\mathbf J_s}
\newcommand{\ms}{\mathbf M_s}

\newcommand{\eneg}{e^{-ik_1z}}
\newcommand{\epos}{e^{ik_1z}}
\newcommand{\ein}{e^{in\phi}}

\def\Deltamur{\Delta\bmu_r}
\def\Deltaepsr{\Delta\beps_r}

\newcommand{\bbarz}{\mathbf{\overline Z}}
\newcommand{\bbarp}{\mathbf{\overline P}}
\newcommand{\bbark}{\mathbf{\overline K}}
\newcommand{\bbara}{\mathbf{\overline A}}
\newcommand{\bbarb}{\mathbf{\overline B}}
\newcommand{\bbard}{\mathbf{\overline D}}
\newcommand{\kayq}{{\mathbf{\overline K}}^{-1}\cdot\mathbf Q}
\def\MHE{electromagnetic equations}

\renewcommand{\v}[1]{{{\bf #1}}}
\def\dyad #1{\v{\overline{#1}}}
\def\braket#1#2{\langle{#1|#2}\rangle}
\def\bra#1{\langle{#1}|}
\def\ket#1{|{#1}\rangle}

\def\gTM{g^{\textrm{\scriptsize TM}}}
\def\gTE{g^{\textrm{\scriptsize TE}}}
\def\gTEs{g_s^{\textrm{\scriptsize TE}}}
\def\gTMr{g^{\textrm{\scriptsize TM}}\left(\v{r},\v{r}'\right)}
\def\gTEr{g^{\textrm{\scriptsize TE}}\left(\v{r},\v{r}'\right)}
\def\gTEsr{g_s^{\textrm{\scriptsize TE}}\left(\v{r},\v{r}'\right)}

\def\gTMS{g^{\textrm{\scriptsize TM},S}}
\def\gTES{g^{\textrm{\scriptsize TE},S}}
\def\gTEsS{g_s^{\textrm{\scriptsize TE},S}}
\def\gTMSr{g^{\textrm{\scriptsize TM},S}\left(\v{r},\v{r}'\right)}
\def\gTESr{g^{\textrm{\scriptsize TE},S}\left(\v{r},\v{r}'\right)}
\def\gTEsSr{g_s^{\textrm{\scriptsize TE},S}\left(\v{r},\v{r}'\right)}

\def\DG{\dyad G}
\def\curl{\nabla\times}
\def\curlp{\nabla'\times}
\def\div{\nabla\cdot}
\def\divp{\nabla'\cdot}
\def\grad{\nabla}
\def\gradp{\nabla'}
\def\curlDG{\curl\DG}

\def\TMS{{{\rm TM},S}}
\def\TES{{{\rm TE},S}}

\def\opL{\mathcal L}
\def\opK{\mathcal K}

\def\kmns{k_{mn}^2}
\def\pr{(\v r)}
\def\prp{(\v r')}
\def\prs{(\vec{r}, \vec{r}')}

\def\prt{(\v r, t)}
\def\prpt{(\v r', t)}

\def\prw{(\v r, \omega)}
\def\prpw{(\v r', \omega)}
\def\prwn{(\v r, \omega_n)}
\def\pw{(\omega)}

\def\rec2pi{\frac1{2\pi}}


\def\DGLM{dyadic Green's function for layered media}


\def\eeqa{\end{eqnarray}}
\renewcommand{\v}[1]{{{\bf #1}}}

\def\unitnormal{\hat{n}}

\def\MHE{electromagnetic equations}
\def\LVS{linear vector space}
\def\IPS{inner product space}
\def\CEM{computational electromagnetics}
\def\be{\begin{equation} }
\def\ee{\end{equation} }
\def\cm{classical mechanics}
\def\qm{quantum mechanics}
\def\EOM{equation of motion}
\def\EsOM{equations of motion}
\def\QM{Quantum mechanics}
\def\SE{Schr\"{o}dinger equation}
\def\Schr{Schr\"{o}dinger}
\def\tr{\text{tr}}
\def\Tr{\text{Tr}}
\def\EMS{effective mass Schr\"odinger}
\def\rep{representation}
\def\EM{electromagnetic}
\def\PBC{periodic boundary condition}
\def\LHS{left-hand side}
\def\RHS{right-hand side}
\def\HO{harmonic oscillator}
\def\DHO{double harmonic oscillator}
\def\RWA{rotating wave approximation}

%End definition of shortcuts for commands;
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%imported from wimmac
%
%The following is from CHEWMAC.TEX

\def\inf{\infty}
\def\intinf{\int\limits_{-\inf}^{\quad\inf}}
\def\intsinf{\int\limits_{0}^{\quad\inf}}
\def\iintinf{\iint\limits_{-\inf}^{\qquad\inf}}
%\def\in #1#2{\int\limits_{#1}^{\quad #2}}
\def\pd #1#2{\frac {\partial #1}{\partial #2}}
\def\krho{k_\rho}
\def\krhoo{k_{\rho 0}}
%\def\v #1{\bf #1}
\def\hg{\hat g}
\def\today{\ifcase\month\or January\or February\or March\or April\or
May\or June\or July\or August\or September\or October\or November\or
December \fi\space\number\day, \number\year}
\def\inf{\infty}%
\def\dbarL{\bar{\bar {L}}}%
\def\degree{$\,^o$ }
\def\bE{{\bf E}}%
\def\tE{\tilde E}
\def\bJ{{\bf J}}%
\def\vr{{\bf r}}%
\def\dG{\bar{\bf G}_o (\vr ,\vr'')}%
\def\sg{g_o(\vr,\vr')}
\def\dbar#1{\bar{\bar{#1}}}%
%\def\dyad#1{\overline {\v #1}}%
%\def\v #1{{\bf #1}}
%\def\frac#1#2{{#1\over#2}}
\def\endeq{\eqno{\ENUM}}
\def\krho{k_\rho}
\def\~{\tilde}
\def\^{\hat}
\def\pd#1#2{\frac{\partial#1}{\partial#2}}


%\def\vg#1{{\bmit { #1}}}
%\def\dyadg#1{\overline {\bmit {#1} }}
\def\R{\Re e}
\def\I{\Im m}
\def\eqn#1{\eqno{\text{#1}}}
\def\cal{\fam2 }
%\TagsOnRight \font\bi=cmbxti10 scaled 1120
\def\lover#1{\buildrel \leftarrow \over {#1}}
\def\PVint{{-}\hskip -13.pt\int\limits}
\def\pvint{{-}\hskip -10pt\int\limits}
\def\m{\multline }
\def\em{\endmultline }


\def\itemitems{\hangindent2\parindent \textindent}
\def\items{\hangindent\parindent \textindent}

\def\MTT{{\it IEEE Trans. Microwave Theory Tech.}  MTT-}
\def\AP{{\it IEEE Trans. Antennas Propagat.}  AP-}
\def\GE{{\it IEEE Trans. Geosci. Remote Sensing}  GE-}
\def\RS{{\it Radio Sci.}  }
\def\EL{{\it Electron. Lett.}  }
\def\ritem{\noindent\hangindent=1.pc\hangafter=1}
\def\eitem#1{\par\noindent\hangindent\parindent\hangafter=1
    \hbox {\bf #1\enspace}\ignorespaces}
\def\q{\quad}
\def\qq{\qquad}
\def\qqq{\qq\q}
\def\qqqq{\qqq\q}

\def\three{\text{$\text{I}\text{I}\text{I}$}}
\def\tinf{\text{\it inf\,}}
\def\math#1{\vphantom{\left(#1\right)}#1}
\def\sqrts#1{ {\sqrt{#1}\,} }
\def\sgn{\,\text{\rm sgn}}


\def\bul{$\bullet$\hskip 1pc}
\def\nl{\vskip \baselineskip}
\def\bitem{\item{\bul}}
\def\subitem#1{\hbox{\hskip 2pc\vtop{\hsize 5.5in\parindent 0pt #1}
\hfil}}
\def\cl#1{\centerline{#1}}
\def\ub#1{\underbar{#1}}
\def\ul#1{\underline{#1}}
\def\Cal#1{{\cal #1}}
\def\Real{\Re e~}
\def\Imag{\Im m~}

\def\Div{\nabla\cdot}
\def\Curl{\nabla\times}
\def\Grad{\nabla}

